A decidable policy language for history-based transaction monitoring

Online trading invariably involves dealings between strangers, so it is important for one party to be able to judge objectively the trustworthiness of the other. In such a setting, the decision to trust a user may sensibly be based on that user's past behaviour. We introduce a specification language based on linear temporal logic for expressing a policy for categorising the behaviour patterns of a user depending on its transaction history. We also present an algorithm for checking whether the transaction history obeys the stated policy. To be useful in a real setting, such a language should allow one to express realistic policies which may involve parameter quantification and quantitative or statistical patterns. We introduce several extensions of linear temporal logic to cater for such needs: a restricted form of universal and existential quantification; arbitrary computable functions and relations in the term language; and a "counting" quantifier for counting how many times a formula holds in the past. We then show that model checking a transaction history against a policy, which we call the history-based transaction monitoring problem, is PSPACE-complete in the size of the policy formula and the length of the history. The problem becomes decidable in polynomial time when the policies are fixed. We also consider the problem of transaction monitoring in the case where not all the parameters of actions are observable. We formulate two such "partial observability" monitoring problems, and show their decidability under certain restrictions.

==> complexity.tex <==
\section{Complexity}

We now consider the complexity of model checking our logic.

\begin{thm}
  Let $\varphi \in \ourLTL$ and $h$ be a history.  The problem of
  deciding whether or not $h \models \varphi$ holds is \textsc{pspace}-complete
  in the size of $h$.
\end{thm}

\begin{pf}
  \ldots\TODO{AB: \textsc{pspace}-hardness: reduce classical case.  In \textsc{pspace}:
    argue that algorithm of previous section uses polynomial space.}
\end{pf}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% ispell-local-dictionary: "british"
%%% End: 


==> definitions.tex <==
\section{Preliminaries}

\TODO{AB: For later: Here we should define some basic notions that
  otherwise clutter the main text.  Things that come to mind are
  \begin{itemize}
  \item variables
  \item substitution
  \item domain of substitution
  \item linear arithmetics
  \item \ldots
  \end{itemize}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% ispell-local-dictionary: "british"
%%% End: 


==> expressiveness.tex <==
\section{Expressiveness}

\TODO{AB: Discuss expressiveness, give examples!}

\ldots

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% ispell-local-dictionary: "british"
%%% End: 


==> extensions.tex <==
\section{Further extensions}

One can obviously extend the logic with more ad hoc features and operators.
We shall refrain from adding too much without a good sense of applications. 
We discuss two natural extensions which are useful and not overly
complicated. 

\subsection{Quantifiers with positive guards}

The quantifiers ($\forall$, $\exists$) discussed so far allow one to talk about individual
predicates in the current world. It is natural to extend this to
quantifiers which can mention more complicated relations between 
individuals in the history. We consider here such an extension while still
maintain decidability. 
We first define the notion of {\em positive guards}, given by the grammar below:
$$
G := p(x_1,\ldots,x_m) \mid  G \land G \mid \prev G \mid \always G \mid \sometime G,
$$
where $p$ is a predicate symbol. We shall write $G(x_1,\ldots,x_n)$ to denote a guard $G'$ with 
$n$ pairwise distinct variables $x_1,\ldots,x_n$, ordered according to their
appearence in $G'$ from left to right. We extend the notion of arity to positive guards,
i.e., the guard $G(x_1,\ldots,x_n)$ in this case has arity $n$. Similarly,
the type of $G(x_1,\ldots,x_n)$ is $\tau_1 \times \cdots \tau_n \rightarrow prop$, where
$\tau_i$ is the type of $x_i.$ 
We now extend the language of formulae to those with universal and existential quantifiers 
with positive guards, written, respectively:
$$
\forall \vec x : G(\vec x). \psi
\hbox{ and }
\exists \vec x : G(\vec x). \psi
$$
where $G(\vec x)$ is a positive guard.

The semantics of quantifiers with positive guards are straightforward to define.
That is,
$$
(h,i) \models \forall (x_1,\ldots,x_n) : G(x_1,\ldots,x_n).~\psi
$$
if and only if 
for all $(a_1,\ldots,a_n)$ such that $(h,i) \models G(a_1,\ldots,a_n)$,
we have 
$$
(h,i) \models \psi[a_1/x_1,\ldots,a_n/x_n].
$$
To show decidability of the model checking problem for this extension, we show
that we need only consider finitely many such $(a_1,\ldots,a_n)$.
Before we prove this, let us first introduce some notations concerning variable mappings.
We denote with $dom(\sigma)$ the {\em domain} of the variable mapping $\sigma$, i.e.,
the set of variables for which the mapping is defined.
Given a mapping $\sigma$ and a finite set of variables $V \subseteq dom(\sigma)$, 
we denote with $\sigma_{\upharpoonright V}$ the mapping $\sigma$ with its 
domain restricted to $V.$

\begin{defn}
Let $G$ be a positive guard and let $V = \{x_1,\ldots, x_n\}$ be the set
of free variables occuring in $G.$ Let $h$ be a history and $i$ an
integer. Then a mapping $\sigma$ is a {\em solution} for the triple 
$(h,i, G)$ if and only if $(h,i) \models G\sigma$ and $dom(\sigma) = V.$
\end{defn}

\begin{lem}
\label{lm:guards}
Let $G$ be a positive guard, let $h$ be a history and $i$ and integer.
Then the set of all solutions for $(h,i,G)$ is finite.
\end{lem}
\begin{pf}
Let $S$ denote the set of solutions for $(h,i,G)$. We show by induction
on the size of $G$ that $S$ is finite.
In the base case, i.e., when $G = p(x_1,\ldots,x_n)$,
$S$ is the set $\{(a_1,\ldots,a_n) \mid p(a_1,\ldots,a_n) \in h_i \}$,
which is finite by definition. 
The inductive cases are treated as follows:
\begin{itemize}
\item Suppose $G = G_1 \land G_2$. Let $V_1$ be the free variables of $G_1$
and $V_2$ the free variables of $G_2$. Obviously $V_1 \subseteq V$ and
$V_2 \subseteq V.$
By induction hypothesis, we have $S_1$ and $S_2$ which are the sets of
solutions for, respectively, $G_1$ and $G_2.$
Let $S'$ be the following set:
$$
S' = \{\sigma \mid \sigma_{\upharpoonright V_1} \in S_1 \hbox{ and }
\sigma_{\upharpoonright V_2} \in S_2 \}.
$$
$S'$ is obviously finite since both $S_1$ and $S_2$ are finite. 
It can be easily shown that $S = S'$ hence $S$ is also finite.

\item Suppose $G = \prev G'$, and $i \leq |h|$ and $i > 1$ (otherwise
it is trivial). By inductive hypothesis, we have $S'$ which is
finite and contains all the solutions of $(h,i-1,G').$
It is easy to see that $S = S'$, hence it is also finite.

\item Suppose $G = \sometime G'$. Since $(h,i,G)$ is solvable,
there must exists an $j$ such that $1 \leq j \leq i$ and
$(h,j,G')$ is solvable. By induction hypothesis, for each of such $j$,
we have a finite set $S_j$ which is the set of solutions for $(h,j,G')$. 
It can be shown that 
$$
S = \bigcup \{S_j \mid 1 \leq j \leq i  \hbox{ and $S_j$ is
the set of all solutions of $(h,j,G')$}  \},
$$
which is finite.

\item Suppose $G = \always G'$. Since $(h,i,G)$ is solvable,
we have that for all $j$ such that $1 \leq j \leq i$,
$(h,j,G')$ is solvable. Then by induction hypothesis, we have for
each such $j$ a finite set of solutions $S_j.$
It is easy to see that
$$
S = \bigcap \{S_j\}_{1\leq j \leq i}
$$
which is finite.
\end{itemize}
\qed
\end{pf}

\begin{thm}
The model checking problem for $\ourLTL$ extended with quantifiers
with positive guards is decidable.
\end{thm}
\begin{pf}
By induction on the size of the semantics judgment $(h,i) \models \psi$ and
Lemma~\ref{lm:guards}.
\qed
\end{pf}

%% We shall abbreviat $\prev \cdots \prev p$, with $n$-occurences of $\prev$,
%% as $\prevn n p.$
%% The semantics of these generalized quantifiers are straightforward to define:
%% \begin{itemize}
%% \item $(h,i) \models \forall (x_1,\ldots,x_n) : \always p.\psi$ iff
%% for all $(a_1,\ldots,a_n)$, if $p(a_1,\ldots,a_n) \in h_j$ for all $j \leq i$,
%% then $(h,i) \models \psi[a_1/x_1, \ldots, a_n/x_n].$

%% \item $(h,i) \models \forall (x_1,\ldots,x_n) : \sometime p.\psi$
%% iff for all $(a_1,\ldots,a_n)$, if $p(a_1,\ldots, a_n) \in h_j$ for some 
%% $j\leq i$, then $(h,i) \models \psi[a_1/x_1, \ldots, a_n/x_n].$

%% \item $(h,i) \models \forall (x_1,\ldots,x_n) : \prevn k p. \psi$
%% iff for all $(a_1,\ldots,a_n)$, if $i - k \geq 1$ and 
%% $p(a_1,\ldots,a_n) \in h_{i-k}$, then $(h,i) \models \psi[a_1/x_1, \ldots, a_n/x_n].$

%% \end{itemize}
%% Existential quantifier $\exists \vec x : G.\psi$ is then defined
%% as $\neg \forall \vec x : G. \neg \psi$. Alternatively, one can define
%% directly existential quantifier using the forcing relation, e.g.,
%% $(h,i) \models \exists (x_1,\ldots, x_n) : \always p.\psi$ iff
%% there exists $(a_1,\ldots,a_n)$ such that $p(a_1,\ldots,a_n) \in h_j$ for
%% all $j \leq i$ and $(h,i) \models  \psi[a_1/x_1, \ldots, a_n/x_n].$
%% It is easy to see that both definitions are equivalent.


{\em Examples: } Going back to the eBay example, we can state a
policy like ``all previous transactions for which the seller
received negative feedbacks have value less than 200 dollars''
concisely as follows:
$$
\forall (t,x,v) : \sometime (pay(t,x,v) \land negative).~ v \leq 200.
$$
This can actually be equivalently stated as 
$$
\always [\forall (t,x,v) : pay. negative \impl v \leq 200],
$$
without using the more general positive guards. 
It may appear that more general quantifier is not needed.


==> tableau.tex <==
\section{A Sequent Calculus for Model Checking}


\newcommand{\idruleone}
  {$(id_1)\qquad
    \mynode{h, i, p(\;\vec{t}\;)}
           {\sat}{},$
   where $p(\vec t) \downarrow ~ \in h_i$
}

\newcommand{\idruletwo}
  {$(id_2)\qquad
    \mynode{h, i, p(\vec t)}
           {\unsat}{}$, 
  where $p(\vec t) \downarrow ~ \not \in h_i$
}

\newcommand{\relationruleone}{
 \urule{$(R_1)$}
       {}
       {$\mynode{h, i, R(\vec t), \Delta}
                {\sat}$}
        $R(\vec t)$ is true
}

\newcommand{\relationruletwo}{
 \urule{$(R_2)$}
       {}
       {$\mynode{h, i, R(\vec t), \Delta}
                {\unsat}$}
        $R(\vec t)$ is false
}

\newcommand{\negrule}{
\urule{$(\neg)$}
      {$\mynode{h, i, \psi}{v}$}
      {$\mynode{h, i, \neg \psi}{\neg v}$}
}

\newcommand{\andrule}{
 \brule{$(\land)$}
       {$\mynode{h, i, \psi_1}
                {v_1}$}
       {$\mynode{h, i, \psi_2}{v_2}$}
       {$\mynode
                {h, i, \psi_1 \land \psi_2, \Delta }
                {v_1 \land v_2}$}
}

%% \newcommand{\orrule}{
%%  \urule{$(\lor)$}
%%        {$\mynode
%%                 {h, i, A, B}
%%                 {\mymark}$}
%%        {$\mynode
%%                 {h(i) \myvdash{i} A \lor B, \Delta}
%%                 {\mymark}$}
%% }

\newcommand{\forallrule}{
 \urule{$(\forall)$}
       {$\mynode
                {h, i, \varphi(\vec t_1)}
                {v_1}
         \qquad \cdots \qquad
         \mynode
                {h, i,\varphi(\vec t_n)}
                {v_n}$}
       {$\mynode
                {h, i, \forall \vec x: p.\varphi(\vec x)}
                {\bigwedge_{i=1}^{n} v_i}$}
        \\ $\qquad$ where $\{p(\vec x) \mid p(\vec x) \in h(i)\}
                     = \{p(\vec t_1), \cdots , p(\vec t_n)\}$
}

%% \newcommand{\existsrule}{
%%  \urule{$(\exists)$}
%%        {$\mynode
%%                 {h(i) \myvdash{i} \varphi(\vec t_1), \Delta}
%%                 {\mymark_1}
%%          \qquad \cdots \qquad
%%          \mynode
%%                 {h(i) \myvdash{i} \varphi(\vec t_n), \Delta}
%%                 {\mymark_n}$}
%%        {$\mynode
%%                 {h(i) \myvdash{i} 
%%                         \exists \vec x:p(\vec x). \varphi(\vec x), \Delta}
%%                 {\mymark := \bigvee_{i=1}^{n}\mymark_i}$}
%%         \\ $\qquad$ where $\{p(\vec x) \mid p(\vec x) \in h(i)\}
%%                      = \{p(\vec t_1), \cdots , p(\vec t_n)\}$
%% }

\newcommand{\sincerule}{
 \urule{$(\since_1)$}
       {$\mynode
                {h,i, \psi_2}
                {v_1}
         \qquad
         \mynode{h,i,\psi_1}{v_2}
         \qquad
         \mynode{h,i-1, \psi_1 \since \psi_2}{v_3}
        $}
       {$\mynode
                {h, i, \psi_1 \since \psi_2}
                {v_1 \lor (v_2\land v_3)}$}
        $i > 1$
}

\newcommand{\sincespecialrule}{
 \urule{$(\since_2)$}
       {$\mynode{h, 1, \psi_2}{v}$}
       {$\mynode
                {h, ,1, \psi_1 \since \psi_2}
                {v}$}
}

\newcommand{\prevrule}{
 \urule{$(\prev_1)$}
       {$\mynode
                {h, i-1, \varphi}
                {v}$}
       {$\mynode
                {h, i, \prev \varphi}
                {v}$}
        $i > 1$
}

\newcommand{\prevspecialrule}{
 \urule{$(\prev_2)$}
       {$\mynode
               {h, 1, \varphi, \Delta }
               {v}$}
       {$\mynode
               {h, 1, \prev \varphi, \Delta }
               {v}$}
}


\paragraph{Question:} 

\begin{description}
\item[Dead ends:] The current semantics says that $\prev B$ is true at
  $h_1$. But then it does not make sense to say that 
  $\{p(1)\} \models \prev p(2)$ and
  $\{p(1)\} \models \prev \lnot p(2)$.

\item[Dead ends:] What is the semantics of $A \since B$ at the world
  $h_1$?  There is no predecessor world so it has to be something like
  $A \since B = B$ at $h_1$? Alternatively, we could allow the
  procedure to try to extend the current history with new worlds and
  check whether current history can be consistently extended to
  satisfy $\varphi$.

\item[Closed World Assumption:] Does $\{p(1)\} \models p(2)$ hold? The
  semantics say ``no'' since $p(2) \in \{p(1)\}$ is false.  But the
  semantics also says that the value of $\{p(1)\} \models \lnot p(2)$
  is ``true'' since $p(2) \in \{p(1)\}$ is false.  But I don't think
  that this is really the intention: to me, $\forall x:p.\lnot q(x)$
  says ``$p(t) \in h_1 \to \lnot q(t) \in h_1$''. That is, should
  negation be treated in a constructive way?

\item[Logic Programming:] If we are going to treat worlds as a
  database of facts and counterfacts then we could take a logic
  programming approach and actually compute answers. That is
  $\{p(1)\} \models p(x)$ returns an answer of $x = 1$.

\end{description}


We define a sequent calculus which can be used as a backwards-search
procedure for checking whether $M \models \varphi$ where $M$ is a
finite list $h_1, \cdots , h_k$ of ``worlds''.

The sequent turnstile $\myvdash{i}$ node contains $h_i$. Some rules
move us from world $i$ to world $i-1$ by explicitly bringing $h(i-1)$
into the antecedent of the sequent.

Each sequent rule ``breaks down'' some compound formula $\varphi$
which is in the current world and moves us along the model while
preserving falsifiability upwards: if the old model falsified
$\varphi$ then the new model will falsify $\varphi$.

Each node is either an $\andnode$ or an $\ornode$ or an $\myendnode$
depending upon the rule that is applied to that node. Each node
carries a ``boolean variable'' called $\mymark$ whose value from
$\{\sat, \unsat\}$ is determined by the $\mymark$-values of its
children either in a ``conjunctive'' way or in a ``disjunctive'' way
depending upon whether the node is an $\andnode$ or an $\ornode$. The
$(id)$ rule causes the node to become and $\myendnode$ and forces the
procedure to backtrack.

There are also rules (not shown) for distributing negation over each
connective on the right. Or we can just use nnf: was not sure which
way you would want to go.

Let $M = h_1.\cdots . h_m$ for some positive $m$.  Then $M \models
\varphi$ iff there is a derivation for the root node
$\mynode{h_m \models \varphi}{\mymark}$ returns a $\mymark$ value
of $\sat$. The maximum depth of the and-or search tree is polynomial
in $\mid M \mid \times \mid \varphi \mid$.


\begin{figure}[t]
  \centering
\begin{tabular}[c]{lll}
\idruleone
\\ \\
\idruletwo
\\ \\
\relationruleone
\\ \\
\relationruletwo
\\ \\
\negrule
\\ \\
\andrule
\\ \\
\forallrule
\\ \\
\sincerule
\\ \\
\sincespecialrule
\\ \\
\prevrule
\\ \\
\prevspecialrule
\\
\end{tabular}
  \caption{Evaluation rules for deciding whether $(h,i) \models \varphi$}
  \label{fig:sequent}
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

